Near-Optimal Algorithm for Directed Expander Decompositions

In this work, we present the first algorithm to compute expander decompositions in an m-edge directed graph with near-optimal time \~O(m). Further, our algorithm can maintain such a decomposition in a dynamic graph and again obtains near-optimal update times. Our result improves over previous algorithms of Bernstein-Probst Gutenberg-Saranurak (FOCS 2020), Hua-Kyng-Probst Gutenberg-Wu (SODA 2023) that only obtained algorithms optimal up to subpolynomial factors. In order to obtain our new algorithm, we present a new push-pull-relabel flow framework that generalizes the classic push-relabel flow algorithm Goldberg-Tarjan (JACM 1988) which was later dynamized for computing expander decompositions in undirected graphs Henzinger-Rao-Wang (SIAM J. Comput. 2020), Saranurak-Wang (SODA 2019). We then show that the flow problems formulated in recent work Hua-Kyng-Probst Gutenberg-Wu (SODA 2023) to decompose directed graphs can be solved much more efficiently in the push-pull-relabel flow framework. Recently, our algorithm has already been employed to obtain the currently fastest algorithm to compute min-cost flows Van den Brand-Chen-Kyng-Liu-Probst Gutenberg-Sachdeva (FOCS 2024). We further believe that our algorithm can be used to speed-up and simplify recent breakthroughs in combinatorial graph algorithms towards fast maximum flow algorithms Chuzhoy-Khanna (SODA 2024), Chuzhoy-Khanna (STOC 2024), Bernstein-Blikstad-Saranurak-Tu (FOCS 2024).

==> abstract_old_and_bold.tex <==


    In \cite{saranurak2019expander}, the first near-optimal algorithm was given to compute and maintain an expander decomposition of an undirected graph $G$, that is a partition $\mathcal{X}$ of the vertex set of $G$, such that every cluster $X \in \mathcal{X}$ has $G[X]$ being a \emph{well-connected} graph and only a small fraction of the edges of $G$ are not in any cluster. While prior to \cite{saranurak2019expander}, almost-optimal algorithms for this problem existed, \cite{saranurak2019expander} stands out for the simplicity, accessibility, and speed of its algorithm. Since, \cite{saranurak2019expander} has had a transformative impact on the field of graph algorithm and served as a building block in some of the most important breakthrough results, e.g. in the recent almost-linear time algorithm to solve the min-cost flow problem \cite{chen2022maximum}.

    In this work, we present the first algorithm to compute and maintain expander decompositions in \emph{directed} graphs in near-optimal time. Our algorithm can be interpreted as a vast generalization and strengthening of the result in \cite{saranurak2019expander}, for example, we can ensure that $\mathcal{X}$ is a partition refining over time if $G$ only undergoes deletions, all while preserving simplicity and accessibility of algorithm and analysis. This is in stark contrast to previous techniques for directed graphs which resulted in cumbersome and involved algorithms \cite{bernstein2020deterministic, hua2023maintaining}.
    
    We believe that our work will popularize the usage of directed expander decompositions, just like \cite{saranurak2019expander} did for undirected graphs, and we hope that our algorithm serves as a building block for a new generation of directed graph algorithms and, in particular, propels a recent research initiative for finding combinatorial almost-linear time min-cost flow algorithms. We point out that recently, significant progress on the latter question has been made as the first combinatorial near-linear time algorithm for negative single-source shortest-paths  \cite{bernstein2022negative}, and a new combinatorial algorithm for bipartite matching \cite{chuzhoy2024faster} were given, the former relying on a decomposition akin to directed expander decompositions, and the latter by explicitly using dynamic directed expander decompositions. Further, several dynamic (directed) graph algorithms already employ dynamic, directed expander decompositions \cite{bernstein2020deterministic, hua2023maintaining}.

==> dump.tex <==

\begin{comment}
\begin{algorithm}[H]
\caption{Expander Pruning}\label{alg:Expander Pruning}
\begin{algorithmic}
\State Let $f_0$ be the flow induced by $\Pi$
\For{$i \leq k$}
\State $P_i \leftarrow P_{i-1}$
\State $(f_i, \ell_i) \leftarrow (f_{i-1}, \ell_{i-1})$
\Repeat 
\State $(S, (f_i, \ell_i)) \leftarrow \text{PruneOrCertify}(G, D_i, \tilde{V} = V(G) \setminus P_i, (f_i, \ell_i, \Delta))$
\State $P_i \leftarrow P_i \cup S$
\Until{$S = \emptyset$}
\EndFor
\end{algorithmic}
\end{algorithm}




\begin{theorem}[Expander Pruning]\label{thm:ExpanderPruning} Let $G=(V, E)$ be a $\phi$-expander with $m$ edges. There is a deterministic algorithm with access to adjacency lists of $G$ such that, given an online sequence of $k \leq \phi m / 10$ edge deletions in $G$, can maintain pruned sets $P, Q \subseteq V$ such that the following property holds. Let $G_i$ and $P_i, Q_i$ be the graph $G$ and the set $P, Q$ after the $i$-th deletion. We have, for all $i$,
\begin{enumerate}
    \item $P_0, Q_0=\emptyset$ and $P_i \subseteq P_{i+1}, Q_i \subseteq Q_{i+1}$,
    \item $\operatorname{vol}_G\left(P_i\right), \operatorname{vol}_G\left(Q_i\right)  \leq \frac{2i}{\phi}$,
    \item $e_{G_i}\left(P_i, V \setminus (P_i \cup Q_{i})\right), e_{G_i}\left(V \setminus (P_i \cup Q_i), Q_i\right) \leq \frac{i}{2}$,
    \item $e_{G_i}(P_i, Q_i) \leq i$
    \item $G_i\left\{V \setminus (P_i \cup Q_i)\right\}$ is a $\phi / 6$-expander.
\end{enumerate}
The total time for updating $\left(P_i\right)_i, \left(Q_i\right)_i$ is $O\left(k \log m / \phi^3\right)$.
\end{theorem}

\begin{algorithm}[H]
\caption{Expander Pruning}\label{alg:Expander Pruning}
\begin{algorithmic}
\For{$i \leq k$}
\State $P_i \leftarrow P_{i-1}, Q_i \leftarrow Q_{i-1}$
\State $(f_i, \ell_i, \Delta_i) \leftarrow (f_{i-1}, \ell_{i-1}, \Delta_{i-1}), (g_i, h_i, \Delta_i) \leftarrow (g_{i-1}, h_{i-1}, \Delta_{i-1})$
\Repeat 
\State $(S, (f_i, \ell_i, \Delta_i)) \leftarrow \text{PruneOrCertify}(G, \tilde{V} = V(G) \setminus (P_i \cup Q_i), (f_i, \ell_i, \Delta_i))$
\State $P_i \leftarrow P_i \cup S$
\State $(T, (g_i, h_i, \Delta_i)) \leftarrow 
\text{PruneOrCertify}(G^{rev}, \tilde{V} = V(G) \setminus (P_i \cup Q_i), (g_i, h_i, \Delta_i))$
\State $Q_i \leftarrow Q_i \cup T$
\Until{$S, T = \emptyset$}
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{proof}[Proof of Theorem \ref{thm:ExpanderPruning}]
    We begin with verifying that we correctly call $\operatorname{PruneOrCertify}$.\\
    \\
    \textbf{Claim:} Given, We have that $(f_{i-1}|_{G_i[V]}, \ell_i)$ is a valid state on $G_i[]$ for 
    \begin{proof}
        
    \end{proof}
    We enumerate the sets $S, T$ by $S_k, T_k$ over all loops. By condition two of Lemma \ref{lm:PruneOrCertify} we obtain, if $S_k, T_k$ belong to the $i$-th iteration of the for-loop.
    \begin{align}
        e_{G_i}\left(S_k, V \setminus \left(\bigcup_{j \leq k} S_j \cup \bigcup_{j \leq k-1} T_j \right)\right) &\leq \frac{\phi}{4} \cdot \text{vol}_G(S_k) \\
        e_{G_i}\left(T_k, V \setminus \left(\bigcup_{j \leq k} S_j \cup \bigcup_{j \leq k} T_j \right)\right) &\leq \frac{\phi}{4} \cdot \text{vol}_G(S_k)
    \end{align}
    Let $S_l, T_l$ be the last sets $S, T$ belonging to the $i$-th iteration. Then, we have 
    \[P_i = \bigcup_{k \leq l} S_k, Q_i = \bigcup_{k \leq l} T_k.\]
    Hence, 
    \begin{align}
        e_{G_i}\left(P_i, V \setminus (P_i \cup Q_{i}) \right) &\leq \sum_{k \leq l} e_{G_i}\left(S_k, V \setminus \left(\bigcup_{j \leq l} S_j \cup \bigcup_{j \leq l} T_j \right)\right) \\
        &\leq \frac{\phi}{4} \cdot \sum_{k \leq l} \text{vol}_G(S_k) = \frac{\phi}{4} \cdot \text{vol}_G(P_i) \label{eq1}
    \end{align}
    and similarly we obtain $e_{G_i}\left(V \setminus (P_i \cup Q_{i} \right), Q_i) \leq \phi \cdot \text{vol}_G(Q_i)$. Moreover, for any edge $e \in E_{G_i}(P_{i}, Q_{i})$ there are $k, j$ such that $e \in E_{G_i}(S_k, T_l)$. If $k \leq j$ then 
    \[e \in E_{G_i}\left(S_k, V \setminus \left(\bigcup_{j \leq k} S_j \cup \bigcup_{j \leq k-1} T_j \right)\right)\]
    and otherwise 
    \[e \in E_{G_i}\left(T_k, V \setminus \left(\bigcup_{j \leq k} S_j \cup \bigcup_{j \leq k} T_j \right)\right).\]
    Hence, 
    \begin{align}
        e_{G_i}(P_i, Q_i) &\leq \sum_{k \leq \ell} e_{G_i}(S_k, V \setminus (P^k \cup Q^{k-1})) + e_{G_i}(V \setminus (P^k \cup Q^{k}), T^{k}) \\
        &\leq \frac{\phi}{4} \cdot (\text{vol}_G(P_i) + \text{vol}_G(Q_i)) \label{eq2}
    \end{align}
    W.l.o.g. we assume that $\text{vol}_G(Q_i) \leq \text{vol}_G(P_i)$. Then inequalities \eqref{eq1}, \eqref{eq2} imply that 
    \[e_{G_i}(P_i, V \setminus P_i) \leq \frac{\phi}{2} \cdot \text{vol}_G(P_i) \]
    Therefore, by Lemma \ref{lm:helper} we have that 
    \[\text{vol}_G(Q_i) \leq \text{vol}_G(P_i) \leq \frac{2i}{\phi}.\]
    Using this bound in turn, we have that inequalities \eqref{eq1}, \eqref{eq2} imply items 3 and 4 of the theorem. Provided the algorithm ExpanderPruning terminates, item 5 follows from condition 1 of Lemma \ref{lm:PruneOrCertify}. It remains to prove that the algorithm terminates and the bound on the run-time.We remark that every time, we invoke PruneOrCertify either the $\ell$ is increased or the pre-flow $f$ was already a feasible flow. Hence, we can bound the run-time of ExpanderPruning by the sum of the run-time for each PruneOrCertify execution. Hence, we obtain the run-time bound
    \[O\left(\sum_{i \leq k} \sum_{v \in V}(\text{ab}_{f_i}(v) + \text{ab}_{g_i}(v) + \Delta_i(v)) \cdot (\ell_{i+1}(v) - \ell_i(v)) \right).\]
    We remark that for any vertex $v: \Delta_i(v), \text{ab}_{f_i}(v), \text{ab}_{g_i}(v)$ are increasing in $i$. Thus, the run-time is bounded by
    \[O\left(\sum_{v \in V}\left((\text{ab}_{f_k}(v) + \text{ab}_{g_k}(v) + \Delta_k(v)) \cdot \sum_{i \leq k} (\ell_{i+1}(v) - \ell_i(v)) \right)\right) = O\left(h \cdot \sum_{v \in V}(\text{ab}_{f_k}(v) + \text{ab}_{g_k}(v) + \Delta_k(v))\right).\]
    Moreover, we remark that
    \[\sum_{v \in V}(\text{ab}_{f_k}(v) + \text{ab}_{g_k}(v)) = O\left(\sum_{v \in V} \Delta_k(v)\right).\]
    Hence, the run-time is bounded by $O(h \cdot \sum_{v \in V} \Delta_k(v)).$ We note that the total source capacity is bounded by
    \begin{align}
        \sum_{v \in V} \Delta_k(v) &= O\left(\frac{4}{\psi} \cdot \text{cong}(\Pi) \cdot (vol_G(P_k \cup Q_k) + |D|)\right) \\
        &= O\left(\frac{|D|}{\phi^2}\right),
    \end{align}
    which yields the bound on the run-time.
\end{proof}

\subsection{Dynamic Expander Decomposition}
\end{comment}


\begin{comment}
\subsection{Expander Pruning}

\begin{lemma} \label{lm:helper}
    Given a $\phi$-expander $G$ and a set of deletions $D$. Then for any sparse cut in $G' = G \setminus D$, we have $\forall S \subseteq V(G'):$
    \[\min\{ e_{G'}(S, V(G) \setminus S), e_{G'}(S, V(G) \setminus S)\}  < \frac{\phi}{2} \cdot \text{vol}_G(S) \longrightarrow vol_G(S) < \frac{2\cdot |D|}{\phi}\]
\end{lemma}

\begin{definition}
    Given a directed graph $G$, a source capacity $\Delta$ and edge capacity $c$, then we call a function $f: E(G) \rightarrow \R$ a pre-flow if 
    \begin{enumerate}
        \item $\forall v \in V(G): \sum_w f(v,w) \leq \sum_u f(u,v) + \Delta(v)$ 
        \item $\forall e=(u,v) \in E(G): f(u,v) \leq c(e)$
    \end{enumerate}
\end{definition}

\begin{lemma}\label{lm:PruneOrCertify}
    Given a $\phi$-expander $G$ with a $\psi$-witness $W$ embedded through $\Pi$ of congestion $\frac{\psi}{\phi}$. For any induced subgraph $G_* = G[\tilde{V}]$ and any set of deletions $D$ in $G$, where $|D| \leq \phi \cdot m$. We denote by $G'_{*} = G_{*} \setminus D$ and $W' = \Pi^{-1}(G_{*}')$. We set edge capacities $c = \frac{2}{\phi}\cdot 1$, sink capacities $\nabla = \deg_W$ and source capacities $\Delta = \frac{4}{\psi}(\deg_{W} - \deg_{W'})$. Then, for any valid-state $(f,\ell)$, the algorithm $\operatorname{PruneOrCertify}$ returns a new valid-state $(f',\ell')$ and a sparse cut $S \subseteq \tilde{V}:$
    \[e_{G'_*}(S,\tilde{V} \setminus S) \leq \frac{\phi}{4} \cdot \text{vol}_G(S).\]
    Moreover, if $S$ is empty the graph is a $\frac{\phi}{6}$-expander. The run time of the algorithm is $O(\sum_{v \in V} (\text{ab}_f(v) + \Delta(v))\cdot \left(\ell'(v) -\ell(v)\right)).$
\end{lemma}

\begin{algorithm}[H]
\caption{PruneOrCertify}\label{alg:PruneOrCertify}
\begin{algorithmic}
\State Compute flow $\boldsymbol{f}'$ by running the Unit Flow algorithm for $h=\frac{16 \log (m)}{\psi \phi}$ rounds on $(\boldsymbol{f}, \ell, \Delta)$.
\If{$\boldsymbol{f}'$ is a feasible flow}
    \State return the state $(f',\ell')$ and the cut $\emptyset$ 
\Else
    \State $S \leftarrow\left\{v \in V(G) \mid\right. \left.\boldsymbol{ex}_{\boldsymbol{f}'}>0\right\}$
\While{$\left|E_{G'_*}(S, V(G) \setminus S)\right| \geq \phi \cdot \text{vol}_{G}(S)$}
\State $S \leftarrow S \cup\left\{v \in V \mid \operatorname{dist}_{(G'_*)_{f'}}(S, v)=1\right\}$
\State return the state $(f',\ell')$ and the cut $S$ 
\EndWhile
\EndIf
\end{algorithmic}
\end{algorithm}

\begin{proof}[Proof of Lemma \ref{lm:PruneOrCertify}]
We claim that if $f'$ is a feasible flow then case 2 occurs and otherwise case 1 occurs. Let us treat these two cases separately.\\
\\
\textbf{Case 1:}
Let us enumerate the sets $S_0 = \{v \in V(G') \mid \boldsymbol{ex}_{\boldsymbol{f}} > 0\}$ and iteratively $S_{i+1} = S_i \cup \{v \in V(G') \mid \text{dist}_{G_{f'}}(S,v) = 1\}$. It suffices to establish the following.\\
\\
\textbf{Claim:} There exists $j \leq h: E_{G''}(S_j,V \setminus S_j) < \phi \cdot vol_{G}(S_j)$

\begin{proof}
    We assume by contradiction that $j$ does not exist. We observe that

    \[vol_{G''}(S_{j+1}) \geq vol_{G''}(S_{j+1}) + e_{G''_{f'}}(S_j, V \setminus S_j)\]

    and that

    \begin{align}
        e_{G''_{f'}}(S_j, V \setminus S_j) &\geq \frac{c \cdot e_{G''}(S_j,V \setminus S_j) - \Delta(S_j)}{c} \\
        &\geq \frac{c \cdot \phi \cdot (\text{vol}_{G''}(S_j) + \text{vol}_{D}(S_j)) - \Delta(S_j)}{c}
    \end{align}
    
\end{proof}

\textbf{Case 2:} Given the feasible flow $f'$, let us construct a new $\frac{\psi}{}$-witness $\tilde{W}$ for the graph $G'_*$ with an embedding $\tilde{\Pi}$ of congestion $\frac{2\psi}{\phi}$ and such that $\forall v \in \tilde{V}: \deg_G(v) \leq \deg_W(v)$. This will verify that $G'_*$ is a $\frac{\phi}{}$-expander.


It is clear that $\Pi_{W' \rightarrow G''}$ is an embedding with congestion $\frac{2\psi}{\phi}$ and it remains to prove the following claim.\\
\\
\textbf{Claim:} $W'$ is a $\frac{\psi}{4}$-expander.

\begin{proof}
    Let us denote $W^0 = \Pi_{W \mapsto G}^{-1}(G'')$.\\
    \\
    Assume by contradiction that there is $S \subseteq W': vol_{W'}(S) \leq vol_{W'}(W' \setminus S)$ such that 
    \[e_{W'}(S, W' \setminus S) \leq \frac{\psi}{4} vol_{W'}(S).\]
    Since $W$ is a $\psi$-expander, we have
    \[e_W(S, W' \setminus S) + e_W(S, W \setminus W') = e_W(S, W \setminus S) \geq \psi \cdot vol_W(S).\]
    In the following, we use these two inequalities to bound the excess source of $S$ by
    \[\Delta(S) > vol_{W}(S) + e_{W'}(S, W' \setminus S),\]
    which yields a contradiction, since the total amount of flow with source in $S$ that can be routed is at most $vol_W(S) + e_{W'}(S, W' \setminus S)$.
    First, we note that
    \[2\deg_W(v) \geq \deg_{W^0}(v) + \deg_W(v) \geq \deg_{W'}(v)\]
    and then obtain
    \begin{align*}
        \Delta(S) &\geq \frac{8}{\psi} (e_W(S, W \setminus W') + (e_W(S, W' \setminus S) - e_{W^0}(S, W' \setminus S))) \\
        &\geq 8vol_W(S) - \frac{8}{\psi} e_{W^0}(S, W' \setminus S) \\
        &\geq 8vol_W(S) - 2 vol_{W'}(S) = 4vol_W(S)\\
        &\geq vol_{W}(S) + e_{W'}(S, W' \setminus S) 
    \end{align*}
    
\end{proof}

    
\end{proof}


\begin{theorem}[Expander Pruning]\label{thm:ExpanderPruning} Let $G=(V, E)$ be a $\phi$-expander with $m$ edges. There is a deterministic algorithm with access to adjacency lists of $G$ such that, given an online sequence of $k \leq \phi m / 10$ edge deletions in $G$, can maintain pruned sets $P, Q \subseteq V$ such that the following property holds. Let $G_i$ and $P_i, Q_i$ be the graph $G$ and the set $P, Q$ after the $i$-th deletion. We have, for all $i$,
\begin{enumerate}
    \item $P_0, Q_0=\emptyset$ and $P_i \subseteq P_{i+1}, Q_i \subseteq Q_{i+1}$,
    \item $\operatorname{vol}_G\left(P_i\right), \operatorname{vol}_G\left(Q_i\right)  \leq \frac{2i}{\phi}$,
    \item $e_{G_i}\left(P_i, V \setminus (P_i \cup Q_{i})\right), e_{G_i}\left(V \setminus (P_i \cup Q_i), Q_i\right) \leq \frac{i}{2}$,
    \item $e_{G_i}(P_i, Q_i) \leq i$
    \item $G_i\left\{V \setminus (P_i \cup Q_i)\right\}$ is a $\phi / 6$-expander.
\end{enumerate}
The total time for updating $\left(P_i\right)_i, \left(Q_i\right)_i$ is $O\left(k \log m / \phi^3\right)$.
\end{theorem}

\begin{algorithm}[H]
\caption{Expander Pruning}\label{alg:Expander Pruning}
\begin{algorithmic}
\For{$i \leq k$}
\State $P_i \leftarrow P_{i-1}, Q_i \leftarrow Q_{i-1}$
\State $(f_i, \ell_i, \Delta_i) \leftarrow (f_{i-1}, \ell_{i-1}, \Delta_{i-1}), (g_i, h_i, \Delta_i) \leftarrow (g_{i-1}, h_{i-1}, \Delta_{i-1})$
\Repeat 
\State $(S, (f_i, \ell_i, \Delta_i)) \leftarrow \text{PruneOrCertify}(G, \tilde{V} = V(G) \setminus (P_i \cup Q_i), (f_i, \ell_i, \Delta_i))$
\State $P_i \leftarrow P_i \cup S$
\State $(T, (g_i, h_i, \Delta_i)) \leftarrow 
\text{PruneOrCertify}(G^{rev}, \tilde{V} = V(G) \setminus (P_i \cup Q_i), (g_i, h_i, \Delta_i))$
\State $Q_i \leftarrow Q_i \cup T$
\Until{$S, T = \emptyset$}
\EndFor
\end{algorithmic}
\end{algorithm}

\begin{proof}[Proof of Theorem \ref{thm:ExpanderPruning}]
    We begin with verifying that we correctly call $\operatorname{PruneOrCertify}$.\\
    \\
    \textbf{Claim:} Given, We have that $(f_{i-1}|_{G_i[V]}, \ell_i)$ is a valid state on $G_i[]$ for 
    \begin{proof}
        
    \end{proof}
    We enumerate the sets $S, T$ by $S_k, T_k$ over all loops. By condition two of Lemma \ref{lm:PruneOrCertify} we obtain, if $S_k, T_k$ belong to the $i$-th iteration of the for-loop.
    \begin{align}
        e_{G_i}\left(S_k, V \setminus \left(\bigcup_{j \leq k} S_j \cup \bigcup_{j \leq k-1} T_j \right)\right) &\leq \frac{\phi}{4} \cdot \text{vol}_G(S_k) \\
        e_{G_i}\left(T_k, V \setminus \left(\bigcup_{j \leq k} S_j \cup \bigcup_{j \leq k} T_j \right)\right) &\leq \frac{\phi}{4} \cdot \text{vol}_G(S_k)
    \end{align}
    Let $S_l, T_l$ be the last sets $S, T$ belonging to the $i$-th iteration. Then, we have 
    \[P_i = \bigcup_{k \leq l} S_k, Q_i = \bigcup_{k \leq l} T_k.\]
    Hence, 
    \begin{align}
        e_{G_i}\left(P_i, V \setminus (P_i \cup Q_{i}) \right) &\leq \sum_{k \leq l} e_{G_i}\left(S_k, V \setminus \left(\bigcup_{j \leq l} S_j \cup \bigcup_{j \leq l} T_j \right)\right) \\
        &\leq \frac{\phi}{4} \cdot \sum_{k \leq l} \text{vol}_G(S_k) = \frac{\phi}{4} \cdot \text{vol}_G(P_i) \label{eq1}
    \end{align}
    and similarly we obtain $e_{G_i}\left(V \setminus (P_i \cup Q_{i} \right), Q_i) \leq \phi \cdot \text{vol}_G(Q_i)$. Moreover, for any edge $e \in E_{G_i}(P_{i}, Q_{i})$ there are $k, j$ such that $e \in E_{G_i}(S_k, T_l)$. If $k \leq j$ then 
    \[e \in E_{G_i}\left(S_k, V \setminus \left(\bigcup_{j \leq k} S_j \cup \bigcup_{j \leq k-1} T_j \right)\right)\]
    and otherwise 
    \[e \in E_{G_i}\left(T_k, V \setminus \left(\bigcup_{j \leq k} S_j \cup \bigcup_{j \leq k} T_j \right)\right).\]
    Hence, 
    \begin{align}
        e_{G_i}(P_i, Q_i) &\leq \sum_{k \leq \ell} e_{G_i}(S_k, V \setminus (P^k \cup Q^{k-1})) + e_{G_i}(V \setminus (P^k \cup Q^{k}), T^{k}) \\
        &\leq \frac{\phi}{4} \cdot (\text{vol}_G(P_i) + \text{vol}_G(Q_i)) \label{eq2}
    \end{align}
    W.l.o.g. we assume that $\text{vol}_G(Q_i) \leq \text{vol}_G(P_i)$. Then inequalities \eqref{eq1}, \eqref{eq2} imply that 
    \[e_{G_i}(P_i, V \setminus P_i) \leq \frac{\phi}{2} \cdot \text{vol}_G(P_i) \]
    Therefore, by Lemma \ref{lm:helper} we have that 
    \[\text{vol}_G(Q_i) \leq \text{vol}_G(P_i) \leq \frac{2i}{\phi}.\]
    Using this bound in turn, we have that inequalities \eqref{eq1}, \eqref{eq2} imply items 3 and 4 of the theorem. Provided the algorithm ExpanderPruning terminates, item 5 follows from condition 1 of Lemma \ref{lm:PruneOrCertify}. It remains to prove that the algorithm terminates and the bound on the run-time.We remark that every time, we invoke PruneOrCertify either the $\ell$ is increased or the pre-flow $f$ was already a feasible flow. Hence, we can bound the run-time of ExpanderPruning by the sum of the run-time for each PruneOrCertify execution. Hence, we obtain the run-time bound
    \[O\left(\sum_{i \leq k} \sum_{v \in V}(\text{ab}_{f_i}(v) + \text{ab}_{g_i}(v) + \Delta_i(v)) \cdot (\ell_{i+1}(v) - \ell_i(v)) \right).\]
    We remark that for any vertex $v: \Delta_i(v), \text{ab}_{f_i}(v), \text{ab}_{g_i}(v)$ are increasing in $i$. Thus, the run-time is bounded by
    \[O\left(\sum_{v \in V}\left((\text{ab}_{f_k}(v) + \text{ab}_{g_k}(v) + \Delta_k(v)) \cdot \sum_{i \leq k} (\ell_{i+1}(v) - \ell_i(v)) \right)\right) = O\left(h \cdot \sum_{v \in V}(\text{ab}_{f_k}(v) + \text{ab}_{g_k}(v) + \Delta_k(v))\right).\]
    Moreover, we remark that
    \[\sum_{v \in V}(\text{ab}_{f_k}(v) + \text{ab}_{g_k}(v)) = O\left(\sum_{v \in V} \Delta_k(v)\right).\]
    Hence, the run-time is bounded by $O(h \cdot \sum_{v \in V} \Delta_k(v)).$ We note that the total source capacity is bounded by
    \begin{align}
        \sum_{v \in V} \Delta_k(v) &= O\left(\frac{4}{\psi} \cdot \text{cong}(\Pi) \cdot (vol_G(P_k \cup Q_k) + |D|)\right) \\
        &= O\left(\frac{|D|}{\phi^2}\right),
    \end{align}
    which yields the bound on the run-time.
\end{proof}

\subsection{Dynamic Expander Decomposition}

\end{comment}
